Shortest Path and Distance Queries on Road Networks: Towards Bridging Theory and Practice

Given two locations $s$ and $t$ in a road network, a distance query returns the minimum network distance from $s$ to $t$, while a shortest path query computes the actual route that achieves the minimum distance. These two types of queries find important applications in practice, and a plethora of solutions have been proposed in past few decades. The existing solutions, however, are optimized for either practical or asymptotic performance, but not both. In particular, the techniques with enhanced practical efficiency are mostly heuristic-based, and they offer unattractive worst-case guarantees in terms of space and time. On the other hand, the methods that are worst-case efficient often entail prohibitive preprocessing or space overheads, which render them inapplicable for the large road networks (with millions of nodes) commonly used in modern map applications. This paper presents {\em Arterial Hierarchy (AH)}, an index structure that narrows the gap between theory and practice in answering shortest path and distance queries on road networks. On the theoretical side, we show that, under a realistic assumption, AH answers any distance query in $\tilde{O}(\log \r)$ time, where $\r = d_{max}/d_{min}$, and $d_{max}$ (resp.\ $d_{min}$) is the largest (resp.\ smallest) $L_\infty$ distance between any two nodes in the road network. In addition, any shortest path query can be answered in $\tilde{O}(k + \log \r)$ time, where $k$ is the number of nodes on the shortest path. On the practical side, we experimentally evaluate AH on a large set of real road networks with up to twenty million nodes, and we demonstrate that (i) AH outperforms the state of the art in terms of query time, and (ii) its space and pre-computation overheads are moderate.

==> 5-Optimizations/optimizations.tex <==
\section{Extensions}\label{sec:exten}
In this section we present two major optimizations for the basic algorithm presented in section ~\ref{sec:details}. The first optimization is called \emph{Node Extension} which more accurately selects transit nodes from the set of local shortest paths in $SelectTransitNode$. The second one is an alternative way of adding shortcuts which greatly improve the query efficiency.

\subsection{Node extension}
In $SelectTransitNode$, we select the transit nodes to $V_i$ by $V_{i-1}$ and $E_{i-1}$. We examine each local shortest path $p\in\mathcal{P}$ to find an edge $e$ that intersects the inner shell. If $e$ is a shortcut, we need to expand $e$ to find the real transit edge contracted by $e$. However, this expansion would probably upgrade a node which is not previously in $V_{i-1}$. As shown in Figure ~\ref{fig:realedge}, $(u',v')$ is the real-edge and is put into $TE_i$. In this case either $u'$ or $v'$ would be selected into $V_i$, but $u'$ or $v'$ is not necessarily in $V_{i-1}$. As a matter of fact, $(u,v)$ could also be considered a transit edge if all the local shortest paths in $\mathcal{P}$ which passes $(u',v')$ also passes $(u,v)$. When we say a path passes a shortcut we mean that the path passes the shortest path contracted by the shortcut. For example, as shown in Figure ~\ref{fig:level2}, when computing $V_2$, we already have four local shortest paths in $\mathcal{P}$: $p_1$ from $v_1$ to $v_3$, $p_2$ from $v_1$ to $v_4$, $p_3$ from $v_2$ to $v_3$ and $p_4$ from $v_2$ to $v_4$. As for $p_3$, the shortcut $(v_9,v_{10})$ contains a real-edge $(v_6,v_{10})$. Since in $\mathcal{P}$ all the shortest path which passes $(v_6,v_{10})$ also passes $(v_9,v_{10})$ (the sub-path $(v_9,v_6,v_{10})$), in this case it is reasonable to take $(v_9,v_{10})$ as an transit edge instead of $(v_6,v_{10})$.

In addition, here we perform a node extension. We consider not only the real-edge $(u',v')$, but a sub-path extended from $u'$ and $v'$. Let $p=(s,\ldots,u,v,\ldots,t)\in\mathcal{P}$ be a local shortest path found by $FindLocalShortestPath$, then $p$ is a path composed of the nodes in $V_{i-1}$, except that neither of its source $s$ nor target $t$ is necessarily in $V_{i-1}$. Let $(u,v)$ be the edge on $p$ that intersects the inner shell of a cell that contains $s$. We further use $(u',v')$ to denote the real-edge contracted by $(u,v)$. If $(u,v)$ is an original edge in $G$, then let $(u',v')=(u,v)$. We extend the sub-path $(u',v')$ on $p$ by $\alpha$ hops ($\alpha$ is a pre-defined parameter), and we call it \emph{$\alpha$-hops extended path from $(u',v')$ of $p$}. For example, if we set $\alpha=2$, we extend the sub-path $(u',v')$ to $(u_1,u,u',v',v,v_1)$, where $u_1$ is the parent of $u$ (on $p$) and $v_1$ likewise. Note that $(u_1,u,v,v_1)$ is a sub-path on $p$, and $(u',v')$ is contracted  by $(u,v)$.  Let $\mathcal{P}_{(u',v')}\subseteq\mathcal{P}$ be the set of local shortest paths that has $(u',v')$ as its real-edge, and the sub-path $p'=(x,\ldots,y)$ be the longest common sub-path among all the $\alpha$-hops extended path from $(u',v')$ on each $p\in\mathcal{P}_{(u',v')}$. Then we put $(x,y)$ as an imaginary transit edge into $TE_i$ although $x$ and $y$ are not really connected by an original edge or shortcut. Further, either $x$ or $y$ would be selected from $TE_i$ as an transit node into $V_i$. In our experiments we select $\alpha=3$, namely, starting from the real-edge $(u',v')$, we trace three hops backward ($u,u_1,u_2$) and tree forward($v,v_1,v_2$). Because we found that the local shortest paths that share the same real-edge would usually diverge at the third hop.

The key point of why Node-extension optimizes the method is that, we chose a longer common sub-path $(x,y)$ shared by a number of local shortest paths instead of the real-edge $(u',v')$ as the candidates of transit edges, which in turns makes the estimation of the node importance more accurate and plausible. This is consistent with our real-life experience. For example, if a path $p'$ is the common sub-path shared by a number of shortest-paths, when planing a route, we would usually pay more attention at the endpoints of $p'$ instead of the middle points. Observe that in this optimization we only substitute the real-edge with a longest common sub-path as a candidate transit edge for selecting transit node. This substitution would not vary the number of transit nodes since the real-edge and the common sub-path cover the same number of local shortest paths.

\subsection{Query indexing}
The second optimization is that, we use an alternative way of adding shortcuts instead of the one described in subsection ~\ref{label{sub:shortcuts}}. After we obtain a partition of nodes into levels $\mathcal{L}=\{L_0,L_1,\ldots,L_h\}$, we impose a total order on the nodes: The nodes in $L_{i+1}$ has a higher rank than those in $L_i$, and within the same level, the node covers more local shortest paths has a higher rank. Now we remove all the shortcuts added before and reconstruct the index in this way: we add two types of shortcuts: \emph{Jumping shortcuts} and \emph{Query shortcuts}. To accelerate the construction of jumping shortcuts, we also add a third type of shortcut \emph{level shortcuts}. Actually not all the level shortcuts are used in the query, hence, after constructing jumping shortcuts, we only preserve a subset of level shortcuts which are useful in the queries, and we call them query shortcuts.

\subsubsection{Jumping shortcuts and query shortcuts}
Before constructing the shortcuts, we slightly adjust the nodes layers. We define $\mathcal{R}=\{R_0,\ldots,R_h\}$, where $R_i=\bigcup\limits_{j=i}^h{R_j}$ for $0\leq i\leq h$, i.e. $R_i$ is the set of nodes that are at least in level $i$. We start from $i=1$ and $E_0=E$. At the $i$th iteration, firstly we impose a grid on $G$. The grid scale is the same as the one imposed before when computing the node levels, i.e. $g_i\times g_i$. For each $v\in R_i$, we use a similar algorithm to compute the layer-i neighbours of $v$ as described in \ref{sub:shortcuts}. For $v\in R_i$, the layer-i neighbours of $v$ refer to those nodes: if for any node $w$ such that $SP(v,w)$ passes at least one node in $R_i$, and $u$ on $SP(v,w)$ is a node in $R_i$ that is closet to $v$, then $u$ is the layer-i neighbour of $v$. The set of edges (or shortcuts) that connect each $v\in R_i$ to its layer-i neighbours is represented as $E_i$, and we call the edges in $E_i$ level shortcuts. Then at the $i+1$th iteration, the computation of the layer-(i+1) neighbours of a node $v\in R_{i+1}$ can reuse the edges in $E_i$ as shown in Figure ~\ref{fig:levelshortcuts}. The level shortcuts in $E_i$ guarantee the connectivity because $V_{i+1}\subseteq V_i$. %For a node $v\in V_{i+1}$, we perform a Dijkstra traversal from $v$, meanwhile we maintain a counter $ufb$ to count the unfinished branches as described in algorithm ~\ref{alg:addshortcuts}. Different from algorithm ~\ref{alg:addshortcuts}, during the traversal, we only visit the nodes in $V_i$. The level shortcuts in $E_i$ guarantee the connectivity because $V_{i+1}\subseteq V_i$.

%\begin{figure}
%\centering
%\includegraphics[width = 3in]{figures/levelshortcuts.eps}
%\caption{Level shortcuts} \label{fig:levelshortcuts}
%\end{figure}

\begin{figure}[t]
%\begin{small}
\begin{minipage}[t]{1.63 in}
\centering
\includegraphics[width = 1.67in]{figures/levelshortcuts.eps}
\vspace{-3.49mm}
\figcapup \caption{Level shortcuts $\quad$} \label{fig:levelshortcuts} \figcapdown
\end{minipage}
\begin{minipage}[t]{1.85 in}
\centering
%\hspace{3mm}
\includegraphics[width = 1.67in]{figures/jumpingshortcut.eps}
\figcapup \caption{Jumping shortcuts $\quad$} \label{fig:jumpingshortcut} \figcapdown
\end{minipage}
%\end{small}
\end{figure}

With the level shortcuts we can construct the jumping shortcuts in this way. Starting with $i=1$, at the $i$th iteration, we impose a grid on $G$ sized of $g_i\times g_i$. For each $s\in V-R_i$, (ATTENTION: or $s\in V-R_{i+1}$??) we add a shortcut to its transit node in $R_i$. Let $C$ be the cell that contains $s$. We consider a sub-graph that overlaps with the outer shell of $C$. Then we build a Dijkstra spanning tree rooted from $s$. During the Dijkstra traversal we only visit the nodes in $R_{i-1}$ connected by the level shortcuts. Then from a leaf node $t$, backtrack the path to its root $s$. Let $u$ on the path be the node in $R_i$ that is closet to $v$, then we add a shortcut from $s$ to $u$, which is called jumping shortcut. Such $u$ exists because the leaf node $t$ is outside the outer shell of $C$, and by definition the local shortest path from $s$ to $t$ would pass a transit node, which would be at least in $L_i$ or even higher level. In a word, a jumping shortcut connects a node to the transit node of its cell as illustrated in Figure ~\ref{fig:jumpshortcuts}.

%\begin{figure}
%\centering
%\includegraphics[width = 3in]{figures/jumpingshortcut.eps}
%\caption{Jumping shortcuts} \label{fig:jumpingshortcut}
%\end{figure}

The query shortcuts preserve a subset of the level shortcuts. For each $v\in R_i$, previously we add a level shortcut from $v$ to its layer-i neighbour $u$.  Now we preserve the shortcut only if $Rank_v<Rank_u$.

Although we present the construction of level shortcuts and jumping shortcuts in two separate processes, these two constructions could be performed at the same time, i.e. at the $i$th iteration, we add level shortcuts that connect the nodes in $R_i$, and jumping shortcuts to the nodes in $R_i$ by the level shortcuts added in the $i-1$th iteration.

\subsubsection{Query method}
Now the query method works in the following way: for a given source $s$ and target $t$, we instantiate two Dijkstra traversal respectively from $s$ and $t$. During the traversal we use two priority queues $Q_f$ and $Q_b$ which respectively maintain the forward search from $s$ and the backward search from $t$. Initially $Q_f$ (resp. $Q_b$) contains $s$ (resp. $t$) only. Then we compute how far it is between $s$ and $t$. Based on the geometrical location of $s$ and $t$, we compute the highest level $l$, such that in the $g_l\times g_l$ scale cell, $t$ is beyond the outer shell of the cell that contains $s$, and in the $g_{l+1}\times g_{l+1}$ level scale, $t$ is inside the outer shell. If $l$ is greater than $l_s$, where $l_s$ is the level of $s$, then we dequeue $s$ and enqueue the transit nodes of $s$ into $Q_f$ by jumping shortcuts at level $l$. As illustrated in Figure ~\ref{fig:jumpingshortcut}, we first reach the transit nodes of $s$ (at level $l$) by jumping shortcuts, because the jumping shortcuts direct the search to the nodes that are highly probable on the right shortest path. After that we can perform a similar bidirectional Dijkstra search as described in section ~\ref{sub:query}. If the level of $s$ is greater than $l$, such that from $s$ there is no jumping shortcut at level $l$, then we can start the Dijkstra traversal from $s$. Since the search would only visit a node with higher rank, and $s$ itself is a node of higher rank, so the search would quickly converge to the node with highest rank in the path.

\subsection{Directed graphs}\label{subsec:directedgraphs} 

==> 7-Conclusions/Conclusions.tex <==
\section{Conclusions}\label{sec:conclusion}

This presents Arterial Hierarchiy (AH), a worst-case efficient index structure for shortest path and distance queries on road networks. Under a practical assumption about the road network, AH offers superior query time complexities in both shortest path and distance queries, and its space and preprocessing time complexities are comparable to the best existing worst-case efficient methods. With extensive experiments on real datasets, we show that AH also provides excellent query efficiency in practice, and it even outperforms CH (i.e., the state-of-the-art heuristic method) in terms of query time. Although AH's space consumption and preprocessing cost are relatively higher than CH's,  
